Estimation from Indirect Supervision with Linear Moments

In structured prediction problems where we have indirect supervision of the output, maximum marginal likelihood faces two computational obstacles: non-convexity of the objective and intractability of even a single gradient computation. In this paper, we bypass both obstacles for a class of what we call linear indirectly-supervised problems. Our approach is simple: we solve a linear system to estimate sufficient statistics of the model, which we then use to estimate parameters via convex optimization. We analyze the statistical properties of our approach and show empirically that it is effective in two settings: learning with local privacy constraints and learning from low-cost count-based annotations.

==> arxiv.tex <==
\section{Asymptotic analysis}
\label{sec:variance}

We have two estimators:
maximum marginal likelihood ($\MargML$),
which is difficult to compute,
requiring non-convex optimization and possibly intractable inference;
and our moments-based estimator ($\MomML$),
which is easy to compute,
requiring only solving a linear system and convex optimization.
In this section, we study and compare the \emph{statistical efficiency}
of $\MargML$ and $\MomML$.
For simplicity, we focus on unconditional setting where $x$ is empty,
and omit $x$ in this section.
We also assume our exponential family model is well-specified and that
$\theta^*$ are the true parameters.  All expectations are taken with respect
to $y \sim p_{\theta^*}$.


Recall from \refeqn{betaGivesMu} that $\E[\beta(o) \mid x] = \phi(y)$.
We can therefore think of $\beta(o)$ as a ``best guess'' of $\phi(y)$.
The following lemma provides the asymptotic variances of the estimators:
\begin{proposition}[General asymptotic variances] 
  \label{prop:variance}
  Let $\sI \eqdef \cov[\phi(y)]$ be the Fisher information matrix.
  Then
  \begin{align*}
    \sqrt{n}(\MargML - \theta^*) \cvd \sN(0, \vMargML) ~~ \mbox{and}\\
    \sqrt{n}(\MomML - \theta^*) \cvd \sN(0, \vMomML),
  \end{align*}
  where the asymptotic variances are
  \begin{align}
    \label{eqn:margVariance}
    \vMargML &= (\sI - \E[\cov[\phi(y) \mid o]])^{-1}, \\
    \label{eqn:momVariance}
    \vMomML &= \sI^{-1} + \sI^{-1} \E[\cov[\beta(o) \mid y]] \sI^{-1}.
  \end{align}
\end{proposition}

Let us compare the asymptotic variances of $\MargML$ and $\MomML$ to that of
the fully-supervised maximum likelihood estimator $\hat{\theta}_{\rm full}$,
which has access to $\{(x^{(i)}, y^{(i)})\}$, and satisfies
$\sqrt{n}(\hat{\theta}_{\rm full} - \theta^*) \cvd \sN(0, \sI^{-1})$.

Examining the asymptotic variance of $\MargML$ \refeqn{margVariance}, we see
that the loss in statistical efficiency with respect to maximum likelihood is the
amount of variation in $\phi(y)$ not explained by $o$, $\cov[\phi(y) \mid o]$.
Consequently, if $y$ is simply deterministic given
$o$, then $\cov[\phi(y) \mid o] = 0$, and $\MargML$ achieves the
statistically efficient asymptotic variance $\sI^{-1}$.

The story with $\MomML$ is dual to that for the marginal
likelihood estimator. Considering the second term in
expression~\eqref{eqn:momVariance}, we see that the loss of efficiency due
to our observation model grows linearly in the variability of the
observations $\beta(o)$ not explained by $y$. Thus, unlike $\MargML$, even
if $y$ is deterministic given $o$ (so $o$ reveals full information about
$y$), we do not recover the efficient covariance $\sI^{-1}$.
As a trivial example, let $\phi(y) = y \in
\{0,1\}$ and the observation $o = [y, y + \eta]^\top$ for $\eta \sim \sN(0, 1)$,
so that $o$ contains a faithful copy of $y$,
and let $\beta(o) = \frac{o[1] + o[2]}{2} = y + \frac{\eta}{2}$. Then
$\E[\cov[\beta(o) \mid y]] = \frac{1}{4}$, and
the asymptotic relative efficiency of $\MomML$ to $\MargML$
is $\frac{1}{1 + \sI^{-1} / 4}$.
Roughly, $\MargML$ integrates posterior information about $y$ better
than $\MomML$ does.



\begin{proof}
To compute $\vMargML$, we follow standard arguments in
\citet{vaart98asymptotic}.  If $\ell(o; \theta)$ is the marginal
log-likelihood, then a straightforward calculation yields $\nabla \ell(o,
\theta^*) = \E[\phi(y) \mid o] - \E[\phi(y)]$.  The asymptotic variance is
the inverse of $\E[\nabla \ell(o, \theta^*) \nabla \ell(o, \theta^*)^\top] =
\cov[\E[\phi(y) \mid o]]$; applying the variance decomposition $\sI =
\cov[\E[\phi(y) \mid o]] + \E[\cov[\phi(y) \mid o]]$
gives~\eqref{eqn:margVariance}.

To compute $\vMomML$, recall that the moments-based estimator computes
$\hat\mu = \hat\E[\beta(o)]$ and $\hat\theta = (\nabla A)^{-1}(\hat\mu)$.
Apply the delta method, where $\nabla (\nabla A)^{-1}(\mu^*) = (\nabla^2
A(\theta^*))^{-1} = \cov[\phi(y)]^{-1}$.  Finally, decompose $\cov[\beta(o)]
= \cov[\E[\beta(o) \mid y]] + \E[\cov[\beta(o) \mid y]]$ and recognize that
$\E[\beta(o) \mid y] = \phi(y)$ to obtain~\eqref{eqn:momVariance}.
\end{proof}

\paragraph{Randomized response.}

To obtain concrete intuition for \refprop{variance},
we specialize to the case where $S$ is the randomized response \refeqn{rr}.
In this setting, 
$\beta(o) = \epsilon^{-1} \phi(o) - h$ for some constant vector $h$.
Recall the supervision model:
$z \sim \text{Bernoulli}(\epsilon)$,
$o = y$ if $z = 1$ and $o = y' \sim u$ if $z = 0$.

\begin{lemma}[asymptotic variances (randomized response)] 
  \label{lem:variancerr}
  Under the randomized response model of \refeqn{rr}, the asymptotic variance
  of $\MargML$ is
  \begin{align}
    \label{eqn:variances-rr}
    \lefteqn{\vMomML = \sI^{-1} + \sI^{-1} H  \sI^{-1},} \\
    H &\eqdef \frac{1-\epsilon}{\epsilon^2}\cov[\phi(y')]
      + \frac{1 - \epsilon}{\epsilon}
      \E[(\phi(y) - \E[\phi(y')])\vecsquare]. \nonumber
  \end{align}
\end{lemma}
The matrix $H$ governs the loss of efficiency, which stems from two sources:
(i) $\cov[\phi(y')]$, the variance when we sample $y' \sim u$; and
(ii) the variance in choosing between $y$ and $y'$.
If $y'$ and $y$ have the same distribution,
then $H = \sI \frac{1 - \epsilon^2}{\epsilon^2}$
and $\vMomML = \epsilon^{-2} \sI^{-1}$.

\begin{proof}
  We decompose $\cov[\beta(o) \mid y]$ as
  \begin{align*}
    \lefteqn{\E[\cov[\beta(o) \mid y, z] \mid y]
      + \cov[\E[\beta(o) \mid y, z] \mid y]} \\
    & = \E[\epsilon \cdot 0
      + (1 - \epsilon) \cov[\epsilon^{-1} \phi(y')]
      \mid y] \\
    & ~~ + \cov[z\epsilon^{-1} \phi(y)
      + (1 - z) \E[\epsilon^{-1}\phi(y')] \mid y] \\
    & = \frac{1 - \epsilon}{\epsilon^2} \cov[\phi(y')]
    + \frac{1 - \epsilon}{\epsilon} (\phi(y) - \E[\phi(y')])\vecsquare,
  \end{align*}
  where we used
  $\beta(y) = \epsilon^{-1}\phi(y) - h$.
\end{proof}


\begin{figure}
  \begin{center}
    \begin{tabular}{cc}
      \hspace{-.4cm}
      \includegraphics[width=.54\columnwidth]{graphics/figures_efficiency_epsilon}
      & \hspace{-.3cm}
      \includegraphics[width=.54\columnwidth]{graphics/figures_efficiency_epsilon2} \\
      (a) & (b)
    \end{tabular}
    \caption{\label{fig:efficiency-rr}
      The efficiency of $\MomML$ relative to $\MargML$ as $\epsilon$ varies
      for weak (a) and strong (b) signals $\theta$.}
  \end{center}
\end{figure}



\paragraph{An empirical plot.}
The H\'ajek-Le Cam convolution and local asymptotic minimax theorems give
that $\MargML$ is the most statistically efficient estimator.  We now
empirically study the efficiency of $\MomML$ relative to $\MargML$, where
$\eff \eqdef d^{-1} \tr(\vMargML \vMomML^{-1})$, the average of the relative
variances per coordinate of $\MargML$ to $\MomML$.  We continue to focus on
randomized response in the unconditional case.


To study the effect of $\epsilon$, we consider the following probability
model: we let $y \in \{1, 2, 3, 4\}$, define
\begin{equation*}
  \phi(1) = \left[\begin{matrix} 0 \\ 0 \end{matrix} \right], ~~
  \phi(2) = \left[\begin{matrix} 0 \\ 1 \end{matrix} \right], ~~
  \phi(3) = \left[\begin{matrix} 1 \\ 0 \end{matrix} \right], ~~
  \phi(4) = \left[\begin{matrix} 1 \\ 1 \end{matrix} \right],
\end{equation*}
and set $p_\theta(y) \propto \exp(\theta^\top \phi(y))$.  We set $\theta =
[2, -0.1]^\top$ and $\theta = [5, -1]^\top$ to represent weak and strong
signals $\theta$ (the latter is harder to estimate, as the Fisher
information matrix is much smaller); when $\theta = 0$, the asymptotic
variances are equal, $\vMomML = \vMargML$. In
Figure~\ref{fig:efficiency-rr}, we see that the asymptotic efficiency of
$\MomML$ relative to $\MargML$ decreases as $\epsilon \to 0$, which is
explained by the fact that---as we see in
expression~\eqref{eqn:margVariance}---the $\MargML$ estimator leverages the
prior information about $y$ based on $\theta^*$, while as $\epsilon \to 0$,
expression~\eqref{eqn:variances-rr} is dominated by the $1 / \epsilon^2
\cov[\phi(y')]$ term, where $y'$ is uniform. Moreover, as $\theta$
grows larger, the conditional covariance $\cov[\phi(y) \mid o]$
is much smaller than the covariance $\cov[\beta(o) \mid y]$,
so that we expect that $\vMargML \preceq \vMomML$.

















